Sociotechnical Implications of Generative Artificial Intelligence for Information Access

Robust access to trustworthy information is a critical need for society with implications for knowledge production, public health education, and promoting informed citizenry in democratic societies. Generative AI technologies may enable new ways to access information and improve effectiveness of existing information retrieval systems but we are only starting to understand and grapple with their long-term social implications. In this chapter, we present an overview of some of the systemic consequences and risks of employing generative AI in the context of information access. We also provide recommendations for evaluation and mitigation, and discuss challenges for future research.

==> 98-positionality.tex <==
\subsection*{Positionality statement}
The authors of this paper are$\dots$


==> 99-ack.tex <==
\subsection*{Acknowledgements}
The authors gratefully acknowledge feedback from$\ldots$
